Noisy Gradient Descent Converges to Flat Minima for Nonconvex Matrix Factorization

Numerous empirical evidences have corroborated the importance of noise in nonconvex optimization problems. The theory behind such empirical observations, however, is still largely unknown. This paper studies this fundamental problem through investigating the nonconvex rectangular matrix factorization problem, which has infinitely many global minima due to rotation and scaling invariance. Hence, gradient descent (GD) can converge to any optimum, depending on the initialization. In contrast, we show that a perturbed form of GD with an arbitrary initialization converges to a global optimum that is uniquely determined by the injected noise. Our result implies that the noise imposes implicit bias towards certain optima. Numerical experiments are provided to support our theory.

==> technical report/Convergence.tex <==
%!TEX root = ./noise.tex
\section{Main Results}\label{main}
We study the algorithmic behavior of our proposed perturbed gradient descent (Perturbed GD) algorithm. 
 We primarily focus on the rank-1 nonconvex matrix factorization.
 We first characterize the landscape of the original problem \eqref{mat_fct_ncvx},
 and show that noise effectively smooths the original problem, yielding a smoothed problem \eqref{mat_fact_eq} with benign landscape.
 We then provide a non-asymptotic convergence analysis of the Perturbed GD, and demonstrate the implicit bias induced by the noise.
 In particular, we consider the case where noise is balanced, see more details in Theorem \ref{thm_main}.
 Due to space limit, we defer all the proofs to the appendix. 

We analyze the landscape of the original problem \eqref{mat_fct_ncvx} and the smoothed problem \eqref{mat_fact_eq}. 
Note that due to the bilinear form in $\cF(x,y)$, we have for  $\alpha \neq 0,$ $\displaystyle\cF\left(\alpha x,\alpha^{-1} y\right)=\cF( x,y).$
%Note that $\cF(x,y)$ is homogenious, that is for any $\alpha \neq 0,$ $$\cF\left(\alpha x,\alpha^{-1} y\right)=\cF( x,y).$$ 
The scaling invariance nature of \eqref{mat_fct_ncvx} results in undesired landscape properties, and makes the 
analysis of first order algorithms particularly difficult.
To facilitate further discussions, below we characterize the landscape of  \eqref{mat_fct_ncvx}.

%This results in a significantly increasing complexity of the landscape, especially the structure for global minima. We have the following lemma to characterize the landscape.
\begin{lemma}[\bf Landscape Analysis]\label{lem_landscape}
The gradients of $\cF$ with respect to $x$ and $y$ take the form:
\begin{align*}
\nabla_{x}\cF(x,y)=(xy^\top-M)y,~
\nabla_{y}\cF(x,y)=(xy^\top-M)^{\top}x.
\end{align*}
Then $\cF$ has two types of stationary points: (i) For any $\alpha\neq 0,$  $\left(\alpha u_*, \alpha^{-1} v_*\right)$ is a global optimum; (ii) For any $x\in \RR^{d_1},y\in\RR^{d_2}$ such that $x^\top u_*=y^\top v_*=0,$   $(x,0)$ and $(0,y)$ are strict saddle.
\end{lemma}

The scaling-invariance leads to infinitely many global optima for \eqref{mat_fct_ncvx}, each taking the form $(\alpha u_*, \alpha^{-1} v_*)$. However,  Lemma \ref{lem_condition_number} shows that  different values of $\alpha$ lead to significantly different local landscape around the global minima.

\begin{lemma}\label{lem_condition_number}
The condition number  of  the Hessian matrix of $\cF$ at the global optimum $(\alpha u_*,\alpha^{-1} v_*)$ is $$\kappa\left(\nabla^2 \cF\left(\alpha u_*,\alpha^{-1} v_*\right)\right)=\max\left\{\alpha^4,\alpha^{-4}\right\}+1.$$
\end{lemma}
\begin{figure*}
\centering
\includegraphics[width=\linewidth]{landscape1}
\vspace{-0.2in}
\caption{ The visualization of objective functions $\cF(x,y)=(1-xy)^2$ and  $\tilde\cF(x,y)$ with $x,y\in \RR$ and $\sigma_1^2=\sigma_2^2=0.0975.$  For $\cF(x,y),$ any $(x,y)$ that satisfies $xy=1$ is a global minimum (as shown in (a)). $\tilde\cF(x,y)$ only has global minima close to $\pm(1,1)$ (as shown in (c)).}\label{fig:landscape}
\vspace{-0.1in}
\end{figure*}
From Lemma \ref{lem_condition_number} we know  that when $|\alpha|$ is extremely large or small, 
 the global minimum $(\alpha u_*, \alpha^{-1} v_*)$ is ill-conditioned (large condition number).
%Large condition number has been known to lead to numerical instability in classical optimization literature \citep{XXX}.
The condition number also relates to the sharp/flat minima in neural networks, which we will discuss in detail in Section \ref{sec_discussion}.
%In addition, it is widely believed that for neural networks, large condition number corresponds a sharp local minima, which often yields poor generalization ability. 
Our previous discussion implies that any global optimum $(x_*, y_*)$  to \eqref{mat_fct_ncvx} will be ill-conditioned if the norm ratio $\norm{x_*}_2/\norm{y_*}_2$ is close to zero or infinity.
To facilitate further discussions, we define the balancedness property as follows.



\begin{definition}[$\gamma$-balancedness]\label{def:balance}
We say that $(x,y)\in(\RR^{d_1},\RR^{d_2})$ is $\gamma-$balanced for some positive number $\gamma$ if  $\norm{x}_2=\gamma\norm{y}_2.$
Informally, we say $(x,y)$ is unbalanced if $\gamma$ is close to zero or infinity, and $(x,y)$ is balanced if $\gamma$ is close to 1.\end{definition}

Our next lemma shows that, in the presence of noise, the smoothed problem  \eqref{mat_fact_eq}  has only balanced optima, and the balancedness is completely determined by the ratio of the variance of the noise injected to the iterates.
\begin{lemma}\label{lem_convolutional}
	We say the noise in the Perturbed GD is $\gamma-$balanced if $\EE\left[\norm{\xi_1}_2^2\right]=\gamma^2\EE\left[\norm{\xi_2}_2^2\right]$. 
	For $\gamma = 1$, we say the noise is balanced.
	For any noise ratio $\gamma>0,$ if we take 
	$\sigma^2=\EE\left[\norm{\xi_1}_2^2\right]=\gamma^2\EE\left[\norm{\xi_2}_2^2\right]\leq \min\{\gamma,1\},$
	\eqref{mat_fact_eq} has two global optima $(\tilde u_*(\gamma),\tilde v_*(\gamma))=\pm\sqrt{\gamma-\sigma^2}\left(u_*,\gamma^{-1}v_*\right)$ and one saddle point $(0,0)$ with  $\lambda_{\min}(\nabla^2 \tilde F(0,0))<0$.
\end{lemma}


%The detailed proof is shown in Appendix \ref{pf_1}.
 We see that  when the noise is $\gamma$-balanced and the noise level is sufficiently small, 
 the global minima of 
 the smoothed problem \eqref{mat_fact_eq} can be arbitrarily close to the $\gamma$-balanced global minima of the original rank-1 matrix factorization problem  \eqref{mat_fct_ncvx}. 
 Compared with Lemma \ref{lem_landscape}, Lemma \ref{lem_convolutional} shows that noise effectively smooths the landscape of the original problem  \eqref{mat_fct_ncvx},  the unbalanced optima (with ill-conditioned Hessian) to \eqref{mat_fct_ncvx} are no longer optima after convolution. 
See Figure \ref{fig:landscape} for  detailed illustration of the landscape for the original problem  \eqref{mat_fct_ncvx}  and the smoothed  problem  \eqref{mat_fact_eq}.


Moreover, one can verify that the saddle point $(0,0)$ of problem \eqref{mat_fact_eq}  enjoys the strict saddle property, i.e., the smallest eigenvalue of Hessian at $(0,0)$ is negative. By the stable manifold theory proposed in \citet{lee2019first},  Perturbed GD with an infinitesimal step size and vanishing noise avoids all the strict saddle points and converges to the global optima, asymptotically. However, this asymptotic result does not provide any finite time guarantee. 

We next present the non-asymptotic convergence analysis of our proposed Perturbed GD algorithm.
Our analysis shows that Perturbed GD has implicit bias  determined by the injected noise. 
Specifically, we consider balanced noise, i.e., 
$\EE\left[\norm{\xi_1}_2^2\right]=\EE\left[\norm{\xi_2}_2^2\right]$,
and show that 
%For simplicity, our analysis considers the case where $\gamma=1.$ That is we want to show that with properly chosen noise ($d_1\sigma_1^2=d_2\sigma_2^2$), 
Perturbed GD converges to the balanced $\pm(u_*,v_*)$ in polynomial time in Theorem \ref{thm_main}.  
 

\begin{theorem}[\bf Convergence Analysis]\label{thm_main}
Suppose  $x_0\in \RR^{d_1},$  $y_0\in \RR^{d_2}.$ For any $\epsilon>0$ and for any $\delta\in(0,1),$  we take 
%$$\sigma^2=\EE\left[\norm{\xi_1}_2^2\right]=\EE\left[\norm{\xi_2}_2^2\right]\leq C_{\sigma}\min\left\{\epsilon,\left(\log(1/\delta)\right)^{-2/3} \right\}$$  
$\sigma^2=\EE\left[\norm{\xi_1}_2^2\right]=\EE\left[\norm{\xi_2}_2^2\right]=\rm{poly}(\epsilon,(\log(1/\delta))^{-1}),$
$$\eta={\rm{poly}}( \sigma,\epsilon, (d_1+d_2)^{-1},(\log{(d_1+d_2)})^{-1},(\log(1/\delta))^{-1}).$$

%$$\eta\leq C_\eta \sigma^{10}\min\left\{\epsilon,\frac{1}{d_1+d_2}\left(\log((d_1+d_2)/\delta)\log(1/\delta)\right)^{-1}\right\},$$ where $C_\sigma$ and $C_\eta$ are some absolute positive constants.   

With probability at least $1-\delta,$ we have $\norm{x_t-u_*}_2\leq \epsilon$ and $\norm{y_t-v_*}_2\leq \epsilon.$ for all $t_1\leq t\leq  T_1= O\left({1}/{\eta^2}\right),$ where
$t_1=O\left(\eta^{-1} \sigma^{-2}\log(1/\eta )\log(1/\delta)\right).$
\end{theorem}
 Theorem \ref{thm_main} differs from the convergence analysis of GD in \citet{du2018algorithmic} in the following aspects: (i) Perturbed GD converges regardless of initializations, while GD requires a random initialization near $(0,0)$; 
 (ii) Perturbed GD guarantees convergence with high probability, while GD converges with only constant probability over randomness of initializations;
  (iii) Perturbed GD converges to the balanced solutions ($\norm{x}_2/\norm{y}_2=1$) while GD only maintains approximate balancedness, i.e.,  $c_0\leq\norm{x}_2/\norm{y}_2\leq C_0$ for some absolute constants $c_0, C_0>0.$ 
 
We provide a proof sketch that contains the essential ingredients of characterizing the convergence, since the proof of Theorem \ref{thm_main} is very technical and highly involved. 
See more details and the proof of technical lemmas in Appendix \ref{pf_2}.

\begin{proof}[Proof Sketch]
The convergence of Perturbed GD consists of  three phases: 
{\bf Phase I}: Regardless of initialization, within polynomial time the noise encourages Perturbed GD to escape from region with undesired landscape (e.g., strict saddle points)  and enter the region with benign landscape.
% the algorithm  from the region with undesired landscape (such as the saddle point) after polynomial time. 
{\bf Phase II}: Perturbed GD drives the loss to zero and approaches the set of global minima $\left\{(x,y)\big|xy^\top=M\right\}.$
%minimizes the objective value and stays near the region $\left\{(x,y)\big|xy^\top=M\right\}.$ 
{\bf Phase III}: After the loss is sufficiently small, 
the injected noise dominates the update, which helps the Perturbed GD to balance $x$ and $y,$ and converge to a balanced optimum.

Before we proceed with our proof, 
we first define some notations. Let $U$ and $V$ denote the linear span of $u_*$ and $v_*$, respectively, i.e.,
$
\cU=\{\alpha_1 u_*:\alpha_1\in\RR\},~~\cV=\{\alpha_1 v_*:\alpha_1\in\RR\}.
$
The corresponding orthogonal complement of $\cU$ (or $\cV$) in $\RR^{d_1}$ (or $\RR^{d_2}$) is denoted as $\cU^\perp$ (or $\cV^\perp$).
Our  analysis considers the convergence of Perturbed GD in $(\cU,\cV)$ and $(\cU^\perp,\cV^\perp),$ respectively. Specifically, we take the following orthogonal decomposition of $x_t$ and $y_t$:
\begin{align*}
x_t&=u_*^\top x_t  u_*+(x_t-u_*^\top x_t   u_*),\\y_t&=v_*^\top y_t   v_*+(y_t-v_*^\top y_t   v_*).
\end{align*}
One can check that $(x_t-u_*^\top x_t   u_*)\in\cU^\perp$ and $(y_t-v_*^\top y_t   v_*)\in \cV^\perp,$ respectively. 
%are the components of $x_t,$ $y_t$ in $\cU^\perp$ and  $\cV^\perp,$ 


\noindent $\bullet$ {\bf Phase I}: Regardless of initializations,
 the following lemma shows that $(x_t-u_*^\top x_t   u_*)$ and $(y_t-v_*^\top y_t   v_*)$ vanish after polynomial time.
\begin{lemma}\label{lem_b_converge}
Suppose  $\norm{x_t}^2_2+\norm{y_t}^2_2\leq 2/\sigma^2$ holds for all $t>0.$ For any $\delta\in(0,1)$  we take 
$$\eta\leq \eta_2=C_4{\sigma^8}\left(\log((d_1+d_2)/\delta)\log(1/\delta)\right)^{-1},$$  where $C_4$ is some positive constant. Then with probability at least $1-\delta,$ we have 
\begin{align*}
\norm{x_t-u_*^\top x_t   u_*}_2^2&\leq  2\eta C_2\sigma^{-2},\\
\norm{y_t-v_*^\top y_t   v_*}_2^2&\leq  2\eta C_2\sigma^{-2}
\end{align*}
for any $\tau_1\leq t\leq T_1= O(1/\eta^2),$ where $\tau_1=O(\eta^{-1}\sigma^{-2}\log(1/\eta)\log(1/\delta))$ and  $C_2=(\sigma^2+1/\sigma^2)(2/\sigma^4+6/d_1+6/d_2+6\sigma^4).$
\end{lemma}
Lemma \ref{lem_b_converge} shows that with an arbitrary initialization, the projection of $x_t$ (and $y_t$) onto $\cU^\perp$ (and $\cV^\perp$) vanishes. 
Thus, we only need to characterize the algorithmic behavior of Perturbed GD in subspace $(\cU,\cV).$  
However, as the projection of $x_t$ (and $y_t$) onto $\cU^\perp$ (and $\cV^\perp$) vanishes,
Perturbed GD can possibly approach the region with undesired landscape, e.g., the small neighborhood around the saddle point.
The next lemma shows that the Perturbed GD will escape such regions within polynomial time.
%However, after Perturbed GD improving the solution in $(\cU^\perp,\cV^\perp),$ we cannot rule out the possibility that the algorithm enters some regions with undesired landscape, e.g., the small neighborhood of the saddle point $(0,0).$  The next lemma guarantees that Perturbed GD will not be trapped in these regions. 

%One of the major difficulty here is how to avoid being trapped in the saddle point $(0,0)$. In fact, this saddle point enjoys the strict saddle property \citep{XXXX} and the noise injected to the gradient can help Perturbed GD escape from the saddle.
\begin{lemma}\label{lem_escape}
Suppose $\norm{x_t-u_*^\top x_t   u_*}_2^2\leq  2\eta C_2\sigma^{-2}$ and $\norm{y_t-v_*^\top y_t   v_*}_2^2\leq  2\eta C_2\sigma^{-2}$ hold for all $t>0.$ For any $\delta\in(0,1),$ we take $\eta\leq\eta_3=C_3\sigma^{12}\left(\log((d_1+d_2)/\delta)\log(1/\delta)\right)^{-1},$ where $C_3$ is some positive constant.
Then with probability at least $1-\delta,$  we have 
\begin{align}\label{eq_escape}
x_{t}^\top u_* v_*^\top y_{t}=x_{t}^\top M y_{t}\geq 1/4,
\end{align}
for all $\tau_2\leq t\leq T_1=O\left({1}/{\eta^2}\right),$ where $\tau_2=O\left(\eta^{-1}\sigma^{-2}\log(1/\eta)\log(1/\delta)\right).$
\end{lemma}
%Note that   by Lemma \ref{lem_landscape}, all the global optima $(x,y)$ satisfy $x^\top M y=1,$ $\norm{x_t-u_*^\top x_t   u_*}_2^2=0,$ $\norm{y_t-v_*^\top y_t   v_*}_2^2=0,$ and the unique saddle point $(0,0)$ satisfies $x^\top M y=0.$ 
Since the saddle point $(x,y)=(0,0)$ satisfies $x^\top M y = 0,$ Lemmas \ref{lem_b_converge} and \ref{lem_escape} together imply that regardless of initializations, Perturbed GD is bounded away from the saddle point  after polynomial time.
 The algorithm then enters Phase II and approaches   the set of global optima $\left\{(x,y)\big|xy^\top=M\right\}.$

%To facilitate our following discussion, we explicitly calculate the expectation of the  perturbed gradient as follows. 
%\begin{align*}
%&\nabla_{x}\EE_{\xi_1,\xi_{2}}\left[\cF(x+\xi_{1},y+\xi_{2})\right]=\nabla_{x}\cF(x,y)+d_2\sigma_2^2x,\\
%&\nabla_{y}\EE_{\xi_{1},\xi_{2}}\left[\cF(x+\xi_{1},y+\xi_{2})\right]=\nabla_{y}\cF(x,y)+d_1 \sigma_1^2 y.
%\end{align*} 
% The algorithm then converges to $(u_*,v_*)$ in the next two phases.
 
 \noindent $\bullet$  {\bf Phase II}:
 % After Phase I, $(x_t,y_t)\approx(x_{t}^\top u_*u_*,v_*^\top y_t v_*)$ is away from the saddle point still away from the region $\left\{(x,y)\big|xy^\top=M\right\}.$ 
 In this phase, $(x_t,y_t)$ is still  away from the region $\left\{(x,y)\big|xy^\top=M\right\}.$ Thus,  $\nabla\cF(x_{t},y_{t})$ dominates the update of Perturbed GD.  Perturbed GD behaves similarly to gradient descent while driving the loss to zero. The next lemma formally characterizes this behavior, showing that $xy^
 \top$ converges to $M.$ %(or equivalently $x_{t}^\top u_* v_*^\top y_{t}$ converges to 1).
 \begin{lemma}\label{lem_loss}
 	Suppose $x_{t}^\top u_* v_*^\top y_{t}\geq\frac{1}{4}$ holds for all $t>0.$ For any $\epsilon>0$ and for any $\delta\in(0,1)$, we choose $\sigma\leq\sigma'_1=C_4\sqrt{\epsilon}$ and take 
 	$\eta\leq \eta_4={C}_5{\sigma^6}\left(\log((d_1+d_2)/\delta)\log(1/\delta)\right)^{-1},$  where $C_4,C_5$  are some positive constants. Then with probability at least $1-\delta,$ we have $$\norm{x_ty_t^\top-M}_{\rm{F}}\leq \epsilon,$$
 	for all $\tau_3\leq t\leq  T_1= O\left({1}/{\eta^2}\right),$ where
 	$\tau_3=O\left(\eta^{-1}\log\frac{1}{\sigma}\log(1/\delta)\right).$
 	\end{lemma}
 
 \noindent $\bullet$  {\bf Phase III}: After Phase II, Perturbed GD enters the region where $x_ty_t^\top\approx M.$ Thus, the noise will dominate the update of  the Perturb GD.
Recall in Lemma \ref{lem_condition_number}, we show that the Hessian of unbalanced optima has a large condition number, hence a small perturbation will significantly change the gradient of the objective.
This implies that the unbalanced optima would be  unstable against the noise, and Perturbed GD will escape from such optima and continue iterating towards the balanced optima. 
% As we discuss earlier, at those unbalanced optima, the Hessian matrix is ill conditioned.  A small perturbation will greatly change the gradient and thus, Perturbed GD continues moving until the optima is balanced.
  %Note that the noise induced terms $d_2\sigma_2^2x$ and $d_1 \sigma_1^2 y$ can be viewed as the gradient of $\cF_{bias}(x,y)=\frac{1}{2}d_2\sigma_2^2\norm{x}_2^2+\frac{1}{2}d_1 \sigma_1^2 \norm{y}_2^2.$ The noise  actually induces  this implicit bias  towards the optima that can minimize $\cF_{bias},$ which leads Perturbed GD to balance $x$ and $y.$ Following this intuition, t
 The next lemma shows that $x_t $  and $y_t $ converge to $u_*, v_*,$ respectively.
\begin{lemma}\label{lem_convergence}
For $\forall\epsilon>0$, suppose $\norm{x_ty_t^\top-M}_{\rm{F}}\leq \epsilon$ holds for all $t>0.$ For any $\delta\in(0,1)$, we choose $\sigma\leq\sigma'_2={C}_6\left(\log(1/\delta)\right)^{-1/3}$ and take 
$\eta\leq \eta_5=C_7\sigma^{10}\epsilon,$  where $C_6, C_7$ are some positive constants. Then with probability at least $1-\delta,$ we have 
\begin{align*}
\norm{x_t -u_*}_2\leq \epsilon,~\norm{y_t-v_*}_2\leq \epsilon,
\end{align*}
for all $\tau_3\leq t\leq  T_1= O\left({1}/{\eta^2}\right),$ where
$\tau_4=O\left(\eta^{-1}\sigma^{-2}\log\eta^{-1}\log(1/\delta)\right).$
\end{lemma}
%o prove Lemma \ref{lem_convergence}, we show that  $(u_*^\top x_t- v_*^\top x_t)^2$ vanishes. The convergence directly follows from these two results. 

With all the lemmas in place, we take $\sigma\leq \min\{\sigma'_1,\sigma'_2\},$ $\eta\leq \min\{\eta_1,\eta_2,\eta_3,\eta_4,\eta_5\}$ and $t_1=\tau_1+\tau_2+\tau_3+\tau_4$, then the claim of Theorem \ref{thm_main} follows immediately.
\end{proof}

\vspace{-0.12in}
\section{Extension to Rank-r Matrix Factorization}\label{sec_extend}
\vspace{-0.1in}
We extend our results to the rank-$r$ matrix factorization, which solves the following problem:
%Our analysis can be possibly extended to the rank-r case, i.e., solving the following problem 
\begin{align}\label{rankr_mf}
\min_{X \in \RR^{d_1 \times r},Y \in \RR^{d_2 \times r}} \cF(X,Y) =  \frac{1}{2}\norm{XY^\top - M}_{\rm{F}}^2,
\end{align}  
where $M\in \RR^{d_1\times d_2}$ is a rank-$r$ matrix. 
 Let $M=A\Sigma B^\top$ be the SVD of $M.$ 
%where $A$ and $B$ are two orthogonal matrix in $\RR^{d_1}$ and $\RR^{d_2}.$ 
Let $U_*=A\Sigma^{\frac{1}{2}}$ and $V_*=B\Sigma^{\frac{1}{2}},$ then $(U_*, V_*)$ is a global minimum for problem \eqref{rankr_mf}.
%One can easily verify that $U_*^\top U_*=V_*^\top V_*=\Sigma.$ 
%Recall that  the trajectory of Perturbed GD can be viewed as that of SGD when solving the following optimization problem
%\begin{align}\label{rankr_eq}
%\min_{X,Y}\tilde\cF(X,Y)=\EE_{\xi_{1},\xi_{2}}\cF(X+\xi_1,Y+\xi_2),
%\end{align}
%where $\xi_{1}\in \RR^{d_1\times r}$  with i.i.d. elements drawn from $N(0,\sigma_1^2)$ and $\xi_{2}\in \RR^{d_2\times r}$ with i.i.d. elements drawn from $N(0,\sigma_2^2).$  
Similar to the rank-1 case, using Perturbed GD to solve problem \eqref{rankr_mf} can be viewed as solving the following smoothed problem:
\begin{align}\label{rankr_eq}
\min_{X,Y}\tilde\cF(X,Y)=\EE_{\xi_{1},\xi_{2}}\cF(X+\xi_1,Y+\xi_2),
\end{align}
where $\xi_{1}\in \RR^{d_1\times r},$ $\xi_{2}\in \RR^{d_2\times r}$ have i.i.d. elements drawn from $N(0,\sigma_1^2)$ and   $N(0,\sigma_2^2),$ respectively.  


%In the analysis, the distance between matrices is measured using the following metric instead of the metric induced  by the Frobenius norm. 
%\begin{align}\label{dist}
%\text{dist}(D_1,D_2)=\min_{R\in \RR^{r\times r}:RR^\top=\cI_r}\norm{D_1-D_2R}_F
%\end{align}
%where $D_1$ and $D_2\in\RR^{d,r}.$ 


 The next theorem shows that the noise in Perturbed GD effectively addresses the scaling invariance issue of \eqref{rankr_mf}.
  The smoothed problem \eqref{rankr_eq} only has balanced global minima.
\begin{theorem}\label{thm_rankr}
Let $\sigma_{\min}(M)$ be the smallest singular value of $M$. Suppose $$\EE\left[\norm{\xi_1}_{\rm{F}}^2\right]=\gamma^2\EE\left[\norm{\xi_2}_{\rm{F}}^2\right]=r\gamma^2\sigma^2,$$ and  $\gamma\sigma^2<\sigma_{\min}(M).$ Then  for $\forall(U,V)\in (\RR^{d_1},\RR^{d_2})$ such that $\nabla\tilde\cF(U,V)=0,$ we have
$U^\top U=\gamma^2 V^\top V.$
Moreover,  denote $(\tilde U,\tilde V)=\left(\sqrt{\gamma} A(\Sigma-\gamma\sigma^2I_r)^{\frac{1}{2}},\gamma^{-1/2}B(\Sigma-\gamma\sigma^2I_r)^{\frac{1}{2}}\right),$ then the set  $\{(\tilde U,\tilde V)R \big|R \in \RR^{r\times r}, RR^\top=R^\top R=I_r \}$ contains all the global optima. All other stationary points are strict saddles, i.e., $\lambda_{\min}\left(\nabla^2 \tilde\cF(U,V)\right)<0.$
%Moreover, for any orthogonal matrix $X\in \RR^{r\times r},$ $(\tilde{U},\tilde{V})$ is the global optima, where
%$$(\tilde U,\tilde V)=\pm\sqrt{\gamma-\gamma^2 d_2\sigma_2^2}(U_*X,\frac{1}{\gamma}V_*X).$$
\end{theorem}
%\begin{proof}
%Please see detailed proof in Appendix \ref{pf_3}.
%\end{proof}


Theorem \ref{thm_rankr} shows that  when noise is balanced, \eqref{rankr_eq}  only has balanced global optima and strict saddle points. 
We can invoke \citet{lee2019first} again and show Perturbed GD with an infinitesimal step size and vanishing noise converges to the balanced global optima, asymptotically. %Moreover, when $d_1\sigma_1^2$ is sufficiently small, \eqref{rankr_eq} has global optima arbitrarily closed to $\pm (\sqrt{\gamma}U_*,\gamma^{-1/2}V_*)$, measured in the metric $\mathrm{dist}_\cR(\cdot, \cdot)$. 
%This implies that our Perturbed GD algorithm asymptotically converges to the global optimum close to $\pm (\sqrt{\gamma}U_*,\gamma^{-1/2}V_*).$ 

Note that compared to the rank-1 case, in addition to scaling invariance, the objective is also rotation invariant, i.e., $\tilde\cF(X,Y)= \tilde\cF(XR,YR),$ where $R\in \RR^{r\times r}$ is an orthogonal matrix. 
Thus, we can only recover $U_*$ and $V_*$ up to a rotation factor.
To establish the non-asymptotic convergence result, the optimization error should be measured by the following metric that is rotation invariant:
\begin{align*}
\mathrm{dist}_\cR(D_1,D_2)=\min_{R\in \RR^{r\times r}:RR^\top=I_r}\norm{D_1-D_2R}_{\rm{F}}.
\end{align*}
However, it is more challenging and involved to handle the complex nature of the distance $\mathrm{dist}_\cR(\cdot, \cdot)$. 
As our results for the rank-1 case already provide insights on understanding the implicit bias of noise, we leave the  non-asymptotic analysis of rank-r matrix factorization for future investigation.

%Because of the usage of distance \eqref{dist}, the proof can be very involved and complicated. We leave it 

% We then have the following result to show that for rank-r case, Perturbed GD can still find balanced optima.
%\begin{theorem}
%Suppose  $X_0\in \RR^{d_1\times r},$  $Y_0\in \RR^{d_2\times r}.$ Let $\sigma_{\min}(M)$ be the smallest singular value of $M$. For $\forall \epsilon>0$ and $\delta\in(0,1),$  we take $\sigma^2=d_1\sigma_1^2=d_2\sigma_2^2=\text{poly}(\sigma_{\min}(M),\epsilon,\log)$  and $\eta$ sufficiently small.   With probability at least $1-\delta,$ we have
%\begin{align}
%\text{dist}\left(\begin{bmatrix} 
% X_t\\
%Y_t 
%\end{bmatrix}, \begin{bmatrix} 
%U_*\\
%V_* 
%\end{bmatrix}\right)\leq \epsilon
%\end{align}
%for all $t_1\leq t\leq  T_1= O\left(\frac{1}{\eta^2}\right),$ where
%$t_1=\text{poly}\left(\max(d_1,d_2),\frac{1}{\epsilon},\log(1/\delta)\right).$
%\end{theorem}
%\begin{proof}[Proof Sketch]
%We write X_t=
%\end{proof}

==> technical report/Discussion.tex <==
%!TEX root = ./noise.tex

\vspace{-0.1in}
\section{Discussions}\label{sec_discussion}
\vspace{-0.1in}
\noindent {\bf Connections to SGD.}
This paper studies the implicit bias of the noise in  nonconvex optimization. 
Direct analysis on SGD is beyond current technical limit due to complex dependencies.
Specifically,  the noise in SGD comes from random sampling of the training data, and heavily depends on the iterate. 
This induces a complex dependency between iterate and the noise, and  makes it difficult to characterize the distribution of the noise.

Our Perturbed GD can be viewed as a close variant of SGD.
Moreover, the noise in Perturbed GD follows Gaussian distribution and is independent of the iterates. Hence, the analysis of Perturbed GD, though still highly non-trivial, is now technically manageable.


\noindent {\bf Biased Gradient Estimator.} Different from SGD,  Perturbed GD implements a biased gradient estimator, i.e., $ \EE_{\xi_{1},\xi_{2}}\nabla\cF(x+\xi_1,y+\xi_2)\neq\nabla\cF(x,y).$ Such biased gradient also appears in training deep neural networks combined with computational heuristics.
%  (e.g., dropout \citep{srivastava2014dropout}, batch normalization \citep{ioffe2015batch}, weight normalization \citep{salimans2016weight}).
 Specifically, \cite{luo2018towards} show that with batch normalization,  the gradient estimator in SGD is  also biased with respect to the original loss. The similarity between this biased gradient and our perturbed gradient is worth future investigation.

%Moreover, existing literature shows that normalization helps control the weight to overcome the vanishing gradient issue. Our theory casts new light on explaining the great improvement brought by this simple technique.  Specifically, since the noise of SGD highly depends on the iterates, normalization indirectly controls the noise level. Thus, SGD will converge to the balanced optima.

\noindent {\bf Extension to Other Types of Noise.} Our work considers Gaussian noise, but can be extended to analyzing other types of noise. For example, we can show  that anisotropic noise will have different smoothing
effects along different directions. The implicit bias will thus depend on the covariance of noise in addition to the noise level. For another example, heavy tailed distribution of noise will affect the probability of the convergence of Perturbed GD. It may be difficult to achieve high probability convergence as we have shown for light tailed distributions.

\noindent {\bf Sharp/Flat Minima and Phase Transition.} 
Lemma \ref{lem_condition_number} shows that the Hessian matrix of an unbalanced global optimum is ill-conditioned, and the landscape around such an optimum is sharp in some directions and flat in others. 
For nonconvex matrix factorization, all the global optima are connected and form a path.
The landscape around the path forms a valley, which is narrow around unbalanced optima and wide around the balanced ones (See Figure \ref{fig:landscape2}).
Our three-phase convergence analysis shows that the Perturbed GD first falls into the valley, and then traverses within the valley until it finds the balanced optima.
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{landscape4}
\caption{ The visualization of objective   $\cF(x,y)=(1-xy)^2.$  All the global optima are connected and form a path. The landscape around the path forms a valley.  Around unbalanced optima, the landscape  is sharp in some directions and flat in others.  Around balanced optima, the landscape only contains flat directions.}
\label{fig:landscape2}
\end{figure}

As we have mentioned earlier, people have shown that the local optima of deep neural networks are also  connected. Thus, the phase transition also provides a new perspective to explain the plateau of training curves after learning rate decay in training neural networks. 
Our analysis suggests that after adjusting the learning rate, the algorithm enters a new phase, where the noise slowly re-adjusts the landscape.
At the beginning of this phase, the loss decreases rapidly due to the reduced noise level.
By the end of this phase, the algorithm falls into a region with benign landscape that is suitable for further decreasing the step size.

\noindent {\bf Related Literature.} 
Implicit bias of noise has also been studied in \citet{haochen2020shape,blanc2020implicit}. However, they consider perturbing labels while our work considers perturbing parameters.
In a broader sense, our work is also related to \citet{li2019towards} which show that the noise scale of SGD may change the learning order of patterns. However, they do not study the implicit bias of noise towards certain optima.




==> technical report/Introduction.tex <==
%!TEX root = ./noise.tex
\section{Introduction}
% DNN important
Nonconvex optimization has been widely adopted in various domains, including  image recognition  \citep{hinton2012deep, krizhevsky2012imagenet}, Bayesian graphical models \citep{jordan2004graphical, attias2000variational}, recommendation systems \citep{salakhutdinov2007restricted}, etc. 
Despite the fact that solving a nonconvex problem is generally difficult, empirical evidences have shown that  simple first order algorithms such as stochastic gradient descent (SGD), are able to solve a majority of the aforementioned nonconvex problems efficiently.
The theory behind these empirical observations, however, is still largely unexplored. 

In classical optimization literature, there have been fruitful results on characterizing the convergence of  SGD to first-order stationary points for nonconvex problems.
However, these types of results fall short of explaining the empirical evidences that SGD often converges to global minima for a wide class of nonconvex problems used in practice. 
More recently, understanding the role of noise in the algorithmic behavior of SGD has received significant attention.
%Recently, the presence of noise is widely believed to be of fundamental importance in the success of SGD. 
For instance, \citet{jin2017escape} show that a perturbed form of gradient descent is able to escape from strict saddle points and converge to second-order stationary points (i.e., local minima).  
\citet{zhou2019towards} further show that noise in the update can help SGD to escape from spurious local minima and converge to the global minima.
We argue that, 
despite all these recent results on showing the convergence of SGD to global minima for various nonconvex problems,  
there is still an important question yet to be addressed.
Specifically, the  convergence of SGD  in the presence of multiple global minima remains uncleared for many important nonconvex problems. 
%However, in the presence of multiple global minima in the nonconvex problem, it is unclear what is the role of noise in the algorithmic behavior of SGD.
For example, for over-parameterized neural networks, it has been shown that the nonconvex objective has multiple global minima \citep{kawaguchi2016deep}, only few of which can yield good generalization.
In addition, \citet{allen2018convergence}  show that for an over-parameterized network,  SGD can converge to a global minimum in polynomial time.
Combining with the empirical successes of training over-parameterized neural networks with SGD, these results strongly advocate that SGD not only can solve the nonconvex problem efficiently, but also implicitly biases towards solutions with good generalization ability.
%On the other hand, SGD has been empirically shown to be very successful in finding a global minima with good generalization ability.
%These empirical evidences clearly indicates that the noise in SGD serves as a fundamental role in choosing certain global minima.
Motivated by this, this paper aims to provide more theoretical insights to the following question:
\begin{center}
\textbf{\emph{Does noise impose implicit bias towards certain minimizer
in nonconvex optimization problems?}}
\end{center}

We answer this question through investigating a simple yet non-trivial problem -- nonconvex matrix factorization,  which serves as an important foundation for a wide spectrum of problems such as matrix sensing \citep{bhojanapalli2016dropping,zhao2015nonconvex,chen2015fast,tu2015low}, matrix
completion \citep{keshavan2010matrix,hardt2014understanding,zheng2016convergence}, and deep linear networks \citep{ji2018gradient, gunasekar2018implicit}. 
Given a matrix $M \in \RR^{d_1 \times d_2} $, the nonconvex matrix factorization aims to solve:
\begin{align}\label{mf_obj}
\min_{X\in \RR^{d_1 \times r},Y \in \RR^{d_2 \times r}} \frac{1}{2}\norm{XY^\top - M}_{\rm{F}}^2.
\end{align}
%which can  also be  viewed as a  training two-layer linear network with identity activation function.
Despite its simplicity, \eqref{mf_obj} possesses several intriguing landscape properties: nonconvexity of the objective, all the saddle points satisfy the strict saddle property, and infinitely many global optima due to scaling and rotational invariance.
%In addition, due to scaling and rotational invariance, \eqref{mf_obj} has infinitely many global minima.
Specifically, for any pair of global optimum $(X^*, Y^*)$, $(\alpha X^*, \frac{1}{\alpha} Y^*)$ and $(X^*R, Y^*R)$ are also global optima for any non-zero constant $\alpha$ and rotation matrix $R \in \RR^{r \times r}$. This is different from symmetric matrix factorization, which only possesses rotational invariance. 
The scaling and rotational invariance also imply that the global minima of \eqref{mf_obj} are connected, a landscape property that is also shared by deep neural networks \citep{nguyen2017loss, draxler2018essentially,nguyen2018loss,venturi2018spurious,garipov2018loss,liang2018understanding,nguyen2019connected,kuditipudi2019explaining}.


Nonconvex matrix factorization  \eqref{mf_obj} has been recently studied by \citet{du2018algorithmic}, with  focus on the algorithmic behavior of gradient descent (GD).
Their results reveal an interesting algorithmic regularization imposed by gradient descent: (i) gradient flow (GD with an infinitesimal step size) has automatic balancing property, i.e., the difference of the squared norm $\norm{X}_{\rm{F}}^2 - \norm{Y}_{\rm{F}}^2$ stays constant during training. (ii) for properly chosen step size, GD converges asymptotically for rank-r case,  linearly for rank-1 case, while maintaining approximate balancing property.
%for rank-r problem, GD with small initialization and  diminishing step size maintains approximate balancing property. (3) for rank-1 problem, GD with small initialization and constant step size converges linearly, and the norm $\norm{X}_{\rm{F}}$ and $\norm{Y}_{\rm{F}}$ remains within a constant factor of each other.
%Their results show that, without explicit regularization, the automatic balancing property of GD effectively imposes an algorithmic regularization to problem  \eqref{mf_obj}.
However, \citet{du2018algorithmic} do not consider any noise in the update, 
%However, the analysis of \citep{du2018algorithmic} highly relies on the fact that there is no noise in the update,
 hence their results  can not provide further theoretical insights on understanding the role of noise when applying first order algorithms to nonconvex problems.


In this paper, we are interested in studying the algorithmic behavior of first order algorithms in the presence of noise.
Specifically, we study a perturbed form of gradient descent (Perturbed GD) applied to the matrix factorization problem  \eqref{mf_obj}, which 
 injects independent noise to iterates, and then evaluates gradient at the perturbed iterates.
Note that our algorithm is different from SGD in terms of the noise.
For our algorithm, we inject independent noise to the iterates $(X_t, Y_t)'s$ and use the gradient evaluated at the perturbed iterates.
The noise of SGD, in contrast, comes from the training sample. As a consequence, the noise of SGD has very complex dependence on the iterate, which is difficult to analyze. See more detailed discussions in Sections \ref{sec_discussion}.


We further analyze the convergence properties of our Perturbed GD algorithm for the rank-1 case.
At the early stage, noise helps the algorithm to escape from regions with undesired landscape, including the strict saddle point.
After entering the region with benign landscape, Perturbed GD behaves similarly to gradient descent, until the loss is sufficiently small.   
At the early stage, noise provides additional explorations that help the algorithm to escape from the strict saddle point.
Then at the  later stage, the noise dominates the update of Perturbed GD, and gradually rescales the iterates to a balanced solution that is uniquely determined by the injected noise.
Specifically, the ratio of the norm $\norm{x_t}_2/\norm{y_t}_2$ is completely determined by the ratio of the variance of noise injected to $(x_t, y_t)$.
To the best of our knowledge, this is the first theoretical result towards understanding the implicit bias of noise in nonconvex optimization problems.
Our analysis  reveals an interesting characterization of the local landscape around global minima, which relates to the sharp/flat minima in deep neural networks \citep{keskar2016large}, and we will further discuss these connections in detail in Section \ref{sec_discussion}.
We believe that investigating the implicit bias of the noise in nonconvex matrix factorization can serve as a fundamental building block for studying stochastic optimization for more sophiscated nonconvex problems, including training over-parameterized neural networks.


\noindent{\textbf{Notations}}: $\mathbf{1}$ Given a matrix $A$, $\tr(A)$ denotes the trace of $A.$ For matrices $A,B\in \RR^{n\times m},$  we use $\inner{A}{B}$ to denote the Frobenius inner product, i.e., $\inner{A}{B}=\tr(A^\top B).$ $\norm{A}_{\rm{F}}=\sqrt{\inner{A}{A}}$ denotes the Frobenius norm of $A.$ $I_d\in \RR^{d\times d}$ denotes the identity matrix. 



==> technical report/Model.tex <==
%!TEX root = ./noise.tex
\section {Model and Algorithm}\label{sec_model}
We first describe the nonconvex matrix factorization problem, and then present the perturbed gradient descent algorithm (Perturbed GD).
For simplicity, we primarily focus on the  rank-1 matrix factorization problem. Extensions to the rank-r case are provided in Section \ref{sec_extend}.
\subsection{ Rank-1 Matrix Factorization}
We consider the following nonconvex optimization problem: 
\begin{align}\label{mat_fct_ncvx}
\min_{x\in\RR^{d_1}, y\in\RR^{d_2}}\cF(x,y)=\frac{1}{2}\|xy^\top-M\|^2_{\rm{F}},
\end{align}
 where $M \in \RR^{d_1\times d_2}$ is a rank-1 matrix and can be factorized as follows:
$\displaystyle
M=u_*v_*^\top,
$
where $u_*\in\RR^{d_1}$, $v_*\in\RR^{d_2}$. Without loss of generality, we assume $\norm{u_*}_2=\norm{v_*}_2=1.$


The optimization landscape of \eqref{mat_fct_ncvx} has been well studied in the previous literature \citep{ge2016matrix, ge2017no, chi2019nonconvex, li2019symmetry}.  
 Because of the bilinear form in  $\cF,$ there exist infinitely many global minima to \eqref{mat_fct_ncvx}, including highly unbalanced ones, i.e.,   $xy^\top=M$ with $\norm{x}_2\gg\norm{y}_2$ or $\norm{x}_2\gg\norm{y}_2$ (see Definition \ref{def:balance}).
In Section \ref{main}, we will show that such unbalancedness essentially implies global minima with a large condition number.
 To address this issue, \citet{tu2015low,ge2017no} propose a regularizer of the form $(\norm{x}_2^2-\norm{y}_2^2)^2$ to balance $\norm{x}_2$ and $\norm{y}_2$.
 Recently,  \citet{du2018algorithmic} show that even without explicit regularization, gradient descent  with small random initialization converges to  balanced solutions with constant probability.
 Yet, all of the previous results assume noiseless updates. 
The algorithmic behavior of first order algorithms with noisy updates remains unclear for the nonconvex matrix factorization problem. 
 
  


\subsection{Perturbed Gradient Descent}
To study the effect of noise, we consider a perturbed gradient descent algorithm (Perturbed GD).
At the $t$-th iteration, we first perturb the iterate $(x_t,y_t)$ with independent Gaussian noise $\xi_{1,t}\sim N(0,\sigma_1^2I_{d_1})$ and $\xi_{2,t}\sim N(0,\sigma_2^2I_{d_2}),$ respectively.
We then update $(x_t, y_t)$ with the gradient evaluated at the perturbed iterates. 
The detail of the Perturbed GD algorithm is summarized in Algorithm \ref{alg:Perturbed GD}.
\begin{algorithm}[H]
    \caption{Perturbed Gradient Descent for Rank-1 Matrix Factorization.}
    \label{alg:Perturbed GD}
    \begin{algorithmic}
    	\STATE{\textbf{Input}: step size $\eta$, noise level $\sigma_1, \sigma_2$, matrix $M \in \RR^{d_1 \times d_2}$, number of iterations $T$.}
	\STATE{\textbf{Initialize}: initialize $(x_0, y_0)$ arbitrarily.}
	\FOR{$t = 0 \ldots T-1$}
	\STATE{Sample $\xi_{1,t}  \sim N(0, \sigma_1^2 I_{d_1})$ and $\xi_{2,t} \sim N(0, \sigma_2^2 I_{d_2})$.}
	\STATE{$\tilde{x}_t = x_t + \xi_{1,t}, ~ \tilde{y}_t = y_t + \xi_{2,t}.$}
	\STATE{$x_{t+1} = x_t - \eta (\tilde{x}_t \tilde{y}_t^\top - M ) \tilde{y}_t.$}
	\STATE{$y_{t+1} = y_t - \eta (\tilde{y}_t \tilde{x}_t^\top - M^\top ) \tilde{x}_t.$}
	\ENDFOR
    \end{algorithmic}
\end{algorithm}
 

\textbf{Smoothing Effect}.
 Using Perturbed GD to solve \eqref{mat_fct_ncvx}  can also be viewed as solving the following stochastic optimization problem:
\begin{align}\label{mat_fact_eq}
\min_{x\in\RR^{d_1}, y\in\RR^{d_2}}\tilde\cF(x,y)=\EE_{\xi_{1},\xi_{2}}\cF(x+\xi_1,y+\xi_2),
\end{align}
where $\xi_{1}\sim N(0,\sigma_1^2 I_{d_1})$ and $\xi_{2}\sim N(0,\sigma_2^2 I_{d_2}).$ 
Throughout this paper, we will refer to problem \eqref{mat_fact_eq} as the smoothed problem.
The expectation in  \eqref{mat_fact_eq} can be viewed as convoluting the objective function with a Gaussian kernel. 
In Section  \ref{main}, we show that this convolution effectively  smooths out  unbalanced optima  and yields a benign landscape. 


\begin{remark}
The use of random noise to convolute with the objective function is also known as randomized smoothing, which is first proposed in \citet{duchi2012randomized}.
\citet{zhou2019towards,jin2017escape} further exploit this effect to explain the importance of noise in helping first order algorithms to escape from strict saddle points and spurious local optima.
\end{remark}







==> technical report/Numerical.tex <==
%!TEX root = ./noise.tex
\section{Numerical Experiments}\label{sec_numerical}

We present numerical results to support our theoretical findings. 
We compare our Perturbed GD algorithm with gradient descent (GD), and demonstrate that Perturbed GD with $\gamma-$balanced noise converges to $\gamma-$balanced optima, while the optima obtained by GD are highly sensitive to initialization and step size.
We also show that the phase transition between Phase II and Phase III is not an artifact of the proof, and faithfully captures the true algorithmic behavior of Perturbed GD. 


\noindent\textbf{Rank-1 Matrix Factorization}.
We first consider the rank-1 matrix factorization problem. 
Without loss of generality, the matrix $M$ to be factorized is given by $M = u_* v_*^\top$, where $u_* = (1, 0, \ldots, 0)\in \RR^{d_1}$ and $v_* = (1, 0, \ldots, 0)\in \RR^{d_2}$, with $d_1 = 20$ and $d_2 = 30$. 
We initialize iterates $(x_0, y_0)$ with $x_0 \sim N(0,\sigma_x^2 I_{d_1}),\  y_0 \sim N(0,\sigma_y^2 I_{d_2})$. 
For all experiments, we use $\gamma$-balanced noise in Perturbed GD. 
Specifically, we choose $\xi_{1,t} \sim N(0, \sigma_1^2 I_{d_1}), \xi_{2,t} \sim N(0, \sigma_2^2 I_{d_2})$. 

\noindent\textbf{(1) Balanced Noise}.
We  consider the case of balanced noise ($\gamma =1$), where we take $\sigma_1 = \sqrt{1.5} \times 0.05$ and $\sigma_2 = 0.05$.
One can verify that $\gamma^2 = {d_1 \sigma_1^2}/{(d_2 \sigma_2^2)}  = 1$.

We first use balanced step size to compare with GD studied in  \citet{du2018algorithmic}.
Specifically, we set $\eta_x = \eta_y = 10^{-2}$ for both Perturbed GD and GD.
We further consider two initialization schemes:
(i) small initializations (which is also adopted in \citet{du2018algorithmic}): $\sigma_x = \sigma_y = 10^{-2}$; (ii) large initializations: $\sigma_x = \sigma_y = 10^{-1}$. 
%We repeat the same experiments for $50$ times and report the results in  Fig. \ref{mainresult}.
Fig. \ref{mainresult}.(a, b, d, e)  summarize the results of $100$ repeated experiments in a box-plot. 
%We summarize the quartiles of squared norm ratios of $100$ runs of the same experiments in Fig. \ref{mainresult}.(a, b, d, e). 
As can be seen, regardless of initializations, Perturbed GD always converges to the balanced optima (Fig. \ref{mainresult}.(a, b)).
In contrast, GD only converges to approximately balanced optima for small initializations (Fig. \ref{mainresult}.(d)), and the large initialization yields a large variance in terms of the balancedness of the obtained solution (Fig. \ref{mainresult}.(e)). 
  \begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{box-rk1.pdf}
    \caption{Perturbed GD with balanced noise (a, b and c), Perturbed GD with unbalanced noise (g) and GD (d,e and f) for the rank-1 matrix factorization problem. (a) and (d) use small initializations ($\sigma_x = \sigma_y = 10^{-2}$) and balanced step size ($\eta_x = \eta_y = 10^{-2}$). (b) and (e) use large initializations ($\sigma_x = \sigma_y = 10^{-1}$) and balanced step size. (c) and (f) use small initializations and unbalanced step size ($\eta_x = 0.5 \eta_y  =5 \times 10^{-3}$).}\label{mainresult}
\end{figure*}


We also use unbalanced step size (different step sizes for updating $x$ and $y$) and compare the convergence properties of Perturbed GD and GD. 
Specifically, we set $\eta_x = 0.5 \eta_y  =5 \times 10^{-3}$ for both Perturbed GD and GD.
We adopt a small initialization scheme, with $\sigma_x  = \sigma_y = 10^{-2}$.
Fig. \ref{mainresult}.(c, f)  summarize the results of $100$ repeated simulations in a box-plot. 
%Fig. \ref{mainresult}.(c, f) summarize the results averaging over $100$ runs of the same experiments.
As can be seen, even with small initializations, GD with unbalanced step size converges to the approximately $\sqrt{0.5}$-balanced optima, instead of the $1$-balanced optima (Fig. \ref{mainresult}.(f)). 
In contrast, Perturbed GD is able to converge to the balanced optima with unbalanced step size (Fig. \ref{mainresult}.(c)). 

Our results suggest that the noise is the most important factor in determining the balancedness of the solutions obtained by Perturbed GD. 

%\vspace{+0.1in}

\noindent\textbf{(2) Unbalanced Noise}.
We run Perturbed GD with unbalanced noise.
%To show the implicit bias of the unbalanced noise, we also run  Perturbed GD with unbalanced noise.
We take $\sigma_1 = \sqrt{0.75} \times 0.05$ and $\sigma_2 = 0.05$ with $\gamma^2 ={d_1 \sigma_1^2}/
{(d_2 \sigma_2^2)}= 0.5$. 
We use a  small initialization: $\sigma_x = \sigma_y = 10^{-2}$, and balanced step size: $\eta_x = \eta_y = 10^{-2}$.
Fig. \ref{mainresult}.(g)  summarizes the results of $100$ repeated simulations in a box-plot.
As can be seen,  for $\gamma \neq 1$, the Perturbed GD converges to the $\gamma$-balanced optima.

%\vspace{+0.1in}
\noindent \textbf{Rank-10 Matrix Factorization}. We then consider rank-10 nonconvex matrix factorization problem. 
The matrix $M$ to be factorized is given by $M = U_* V_*^\top$, where 
$
   U_* =\begin{pmatrix}
I_{10}, 0
\end{pmatrix}_{d_1\times10}^\top,
 V_* =\begin{pmatrix}
I_{10}, 0
\end{pmatrix}_{d_2\times10}^\top,
$
with $d_1 = 20$ and $d_2 = 30$. 
We initialize iterates $(X_0, Y_0)$ with all entries ${X_0}^{(i,j)}$'s and ${Y_0}^{(i,j)}$'s independently sampled from $N(0,\sigma_x^2)$ and $N(0,\sigma_y^2)$, respectively.   
%${X_0}^{(i,j)}{\sim} N(0,\sigma_x^2),  {Y_0}^{(i,j)} \sim N(0,\sigma_y^2)$. 
For all experiments, we use $\gamma$-balanced noise in Perturbed GD. 
Specifically, we choose  $\xi_{1,t}$ and $\xi_{2,t}$  with i.i.d. elements drawn from $N(0,\sigma_1^2)$ and $N(0,\sigma_2^2)$ respectively.
We repeat a similar set of experiments as in rank-1 case, and summarize the results in Fig. \ref{mainresultrk-10}.
For each of the experiments, we use the same set of $(\eta_x, \eta_y, \sigma_x, \sigma_y)$ as their counterpart in the rank-1 case.
As can be seen, Perturbed GD always converges to the $\gamma-$balanced optima, regardless of initializations. Our experiments suggest that, for  the  rank-r matrix factorization problem, the noise still determines the balancedness of the optima obtained by Perturbed GD. 
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{box-rk10.pdf}
    \caption{Perturbed GD with balanced noise (a, b and c) and GD (d,e and f) for rank-10 matrix factorization problem. (a) and (d) use small initializations ($\sigma_x = \sigma_y = 10^{-2}$) and balanced step size ($\eta_x = \eta_y = 10^{-2}$). (b) and (e) use large initializations ($\sigma_x = \sigma_y = 10^{-1}$) and balanced step size. (c) and (f) use small initializations and unbalanced step size ($\eta_x = 0.5 \eta_y  =5 \times 10^{-3}$).}\label{mainresultrk-10}
\end{figure*}


\noindent \textbf{Phase Transition.} We further demonstrate the transition between Phase II and Phase III in the Perturbed GD algorithm. Specifically, we consider 2-dimensional problem $f(x,y) = (1-xy)^2$ with balanced optima $\pm(1,1)$. 
We set $\sigma_1 = \sigma_2 = 0.05$, initialize $(x_0 ,y_0) = (3,5)$, and use balanced step size $\eta_x = \eta_y = 0.01$.
We repeat the experiments $50$ times and summarize the result of one realization in Fig. \ref{2phase}, as the convergence properties of Perturbed GD are highly consistent across different realizations.
We also use exponential moving average to smooth the loss trajectory to better illustrate the overall progress of the objective in Phase III.


As can be seen, in around the first $30$ to $40$ iterations,
Perturbed GD and GD behave similarly. 
 Both  Perturbed GD and GD iterate towards the set of global optima $\{(x,y)\big| xy=1\}$, while driving the loss to zero, and the squared norm ratio $x_t^2/y_t^2$ in Perturbed GD decreases from $0.36$ to around $0.004$.
 \begin{figure}[t]
\includegraphics[width=0.9\linewidth]{phase.pdf}
  \caption{Algorithmic behaviors of Perturbed GD and GD. For Perturbed GD, phase transition happens around the first $30\!\sim\!40$ iterations, as shown in (a,b,c). GD does not show phase transitions.  }\label{2phase}
\end{figure}
%Note that during this phase, the noise does not exhibit effect of choosing certain global optimum.
%The GD then converges to unbalanced optimum.
After that, GD converges to the unbalanced optimum. Since the loss is sufficiently small, the noise dominates the update of Perturbed GD.
Then the squared norm ratio $x_t^2/y_t^2$ gradually increases from $0.004$ to $1$.
Perturbed GD  iterates towards the balanced optimum while staying  close to  global optima. 

The phase transition phenomenon can also been observed for higher dimensional problems. As shown in Figure \ref{fig:addit} for $d=4$,  the loss greatly decreases to  and stay around $10^{-4}$   in the first $2\times10^3$ iterations, and then the squared norm ratio ${\norm{x}_2^2}/{\norm{y}_2^2}$ gradually increases from $0.5$ to $1$. This implies the transition between Phase II and Phase III, that is Perturbed GD first approaches the set of global minima and then converges to the balanced optimum. 
\begin{figure}[t]\label{fig:addit}
\includegraphics[width=0.48\linewidth]{PGD_loss.pdf}
\includegraphics[width=0.465\linewidth]{PGD_ratio.pdf}

  \caption{Algorithmic behaviors of Perturbed GD and GD for $d=4$. For Perturbed GD, phase transition happens around the first $2\times10^3$ iterations.  }
\end{figure}

 



==> technical report/abstract.tex <==
%!TEX root = ./noise.tex
\begin{abstract}
%Numerous empirical evidences have corroborated the importance of noise in effective and efficient training of neural networks.
Numerous empirical evidences have corroborated the importance of noise in nonconvex optimization problems.
The theory behind such empirical observations, however, is still largely unknown. 
This paper studies this fundamental problem through investigating the nonconvex rectangular matrix factorization problem, which has infinitely many global minima due to rotation and scaling invariance.
Hence, gradient descent (GD) can converge to any optimum, depending on the initialization. 
In contrast, we show that a perturbed form of GD with an arbitrary initialization converges to a global optimum that is uniquely determined by the injected noise. 
Our result implies that the noise imposes implicit bias towards certain  optima.
Numerical experiments are provided to support our theory.
\end{abstract}
